Sprites and State Channels: Payment Networks that Go Faster than Lightning

Bitcoin, Ethereum and other blockchain-based cryptocurrencies, as deployed today, cannot scale for wide-spread use. A leading approach for cryptocurrency scaling is a smart contract mechanism called a payment channel which enables two mutually distrustful parties to transact efficiently (and only requires a single transaction in the blockchain to set-up). Payment channels can be linked together to form a payment network, such that payments between any two parties can (usually) be routed through the network along a path that connects them. Crucially, both parties can transact without trusting hops along the route. In this paper, we propose a novel variant of payment channels, called Sprites, that reduces the worst-case "collateral cost" that each hop along the route may incur. The benefits of Sprites are two-fold. 1) In Lightning Network, a payment across a path of $\ell$ channels requires locking up collateral for $\Theta(\ell\Delta)$ time, where $\Delta$ is the time to commit an on-chain transaction. Sprites reduces this cost to $O(\ell + \Delta)$. 2) Unlike prior work, Sprites supports partial withdrawals and deposits, during which the channel can continue to operate without interruption. In evaluating Sprites we make several additional contributions. First, our simulation-based security model is the first formalism to model timing guarantees in payment channels. Our construction is also modular, making use of a generic abstraction from folklore, called the "state channel," which we are the first to formalize. We also provide a simulation framework for payment network protocols, which we use to confirm that the Sprites construction mitigates against throughput-reducing attacks.

==> sections/comparisons.tex <==


%\begin{table*}
%\centering
%\makebox[0pt][c]{\parbox{0.9\textwidth}{%
%    \begin{minipage}[b]{0.6\hsize}\centering
%  %\caption{Number of signatures required in each step for the Payment Channels. We use $\times 2$ to highlight if both parties need to co-operate. $d$ is the number of nodes in the branch of Duplex's Invalidation Tree, $\alpha$ is the subset of nodes in the branch of Duplex's Invalidation Tree that need to be resigned, and $\beta$ represents each conditional transfer that is unlocked on-chain.}
%  \caption{A comparison on the number of signatures required for each stage.
%	       Both parties signing the same transaction is represented as $\times 2$, 
%	       The number of nodes that need signed in Duplex's invalidation tree is represented by $d$, and a subset of nodes as $\alpha$. 
%	       The number of conditional transfers that need to be signed and unlocked is represented as $\beta$.  
%           $\times 2$ represents both parties signing the same transaction.   }\label{sigs}
%  \vspace{25pt}
%  \small
%  \begin{tabular}{c|c|c|c|c|c} &
%    \begin{rotate}{30} Establishment \end{rotate} &
%    \begin{rotate}{30} Payment \end{rotate} &
%    \begin{rotate}{30} HTLC \end{rotate} &
%    \begin{rotate}{30} Reset \end{rotate} &
%    \begin{rotate}{30} Dispute \end{rotate} \\
%\hline
%Duplex & $(d + 2) \times 2 $ & $1$ & $1$ & $(\alpha + 1) \times 2$ & $1 \times 2$  \\
%Lightning & $2 \times 2$  & $1 \times 2$ & $1 \times 2$ & N/A & $3$ or $\beta + 3$  \\
%Raiden  & $1$ or $2$   & $1$ & $1$ & N/A & $\beta + 2$  \\ 
%\textbf{Sprite}  & \textbf{1 or 2}  & \textbf{1 $\times$ 2}  & \textbf{1 $\times$ 2} & \textbf{N/A} & \textbf{1}  \\
%  \end{tabular}
%    \end{minipage}
%    \hfill
%    \begin{minipage}[b]{0.35\hsize}\centering
%  \centering
%    \caption{Features Supported by Payment Channels}
%    \small
%    \vspace{25pt}
%   \begin{tabular}{c|c|c|c} &
%      \begin{rotate}{30} Storage \end{rotate} &
%      \begin{rotate}{30} Worst-case delay \end{rotate} &
%      \begin{rotate}{30} Incremental \end{rotate} \\
%  \hline
%  Lightning & 0 & $O(\ell\Delta)$ & \Circle \\
%  Duplex &  0 & \Circle \\
%  Raiden & 0 & $O(\ell\Delta)$ & \Circle \\
%  Sprite & 0 & $O(\ell + \Delta)$ & \CIRCLE \\
%    \end{tabular}
%    \end{minipage}
%    \hfill
%}}
%\end{table*}

\section{Analysis}

In this section, we compare Lightning Channels, Duplex Micropayment Channels, Raiden and Sprite.
All comparisons are based on the protocol descriptions presented in Appendix \ref{survey}. 
We focus on the lock times required to atomically route payments across two or more channels and the number of signatures/transactions required for each step in the protocols. 



\subsection{Lock Times} 

Lightning, Duplex and Raiden have adopted Hashed Time-Locked Contract (HTLC) for conditional transfers that atomically route coins across two or more channels. 

Notably, in a conditional transfer each intermediary party has two roles as the receiver in an incoming channel, and the sender in an outgoing channel. 
Coins are locked into the conditional transfer for $\Delta_{delay}$ blocks which represents the worst-case time that each party must wait before raising a dispute with the Blockchain which is highlighted in Table \ref{features}. 
Cruically, the party must ensure the conditional transfer's expiry time for the incoming channel is greater than the expiry time for the outgoing channel's locked transfer such that $\Delta^{in}_{delay} > \Delta^{out}_{delay}$.
This provides a grace period for this party's coins to be claimed in the outgoing channel before claiming their coins in the incoming channel.

Unfortunately, the worst-case delay $\Delta_{delay}$ in Duplex must take into account the expiry for both the incoming and outgoing channel's lifetime.
This is necessary as disputes cannot be settled in the Blockchain until these channels have expired. 
The worst-case scenario is if the final receiver's channel has the largest expiry time.
In this situation, all hop's along the route's must have a worst-case delay $\Delta_{delay}$ greater than the final channel's expiry time. 

In Lightning and Raiden the worst-case delay $\Delta_{delay}$ only relies on the hop's desired grace period as the channels have no expiry time. 
Although, the sender that establishes the route must lock their coins into the transfer with a lock time greater than the lock times used by all hops along the route.
Ultimately, the coins can be locked for up to $O(\ell\Delta)$ blocks. 
For example, if the worst-case delay $\Delta_{delay}$ is 6 for a route of 10 channels, then the sender's coins are potentially locked for at most 60 blocks. 

The introduction of a Preimage Manager in \textbf{Sprite improves the worst-case delay $\Delta_{delay}$ such that as it remains constant regardless of the route's size}. 
This is possible as Sprite can enforce the success of all conditional transfers along the route if the pre-image $x$ of the conditional hash $H(x)$ is stored in the appointed Preimage Manager's contract before the worst-case delay $\Delta_{delay}$. 
To put another way, any hop can raise a dispute by submitting the pre-image with confidence that all hops along the route will atomically accept the conditional transfer. 
As such, the worst case for the length of time coins are locked into the transfer is $O(\ell + \Delta)$ 

\subsection{Signatures and Transactions} 

Table \ref{sigs} highlights the number of signatures required for each stage of Duplex, Lightning, Raiden and Sprite. 
Next, we provide a comparison on the number of signatures  and the number of transactions that are stored in the Blockchain for each stage of the protocols. 

\textbf{Channel Establishment.} Lightning and Duplex require both parties to sign the channel's state before co-operatively signing a Funding Transaction that is stored in the Blockchain.
In Lighting the state is simply a pair of Commitment Transactions, while in Duplex the state is the first branch of an Invalidation Tree which consists of $d$ nodes and both Unidirectional Channels. 
On the other hand, both Raiden and Sprite require a single party to sign a transaction to establish the channel with their deposit. 
The counterparty can sign a second transaction that deposits their coins into the channel. 

\textbf{Payment.} 
All payments and conditional transfers follow the same approach. 
No additional signatures are required in any scheme to lock coins into a new conditional transfer.
 
Raiden and Duplex are constructed using a pair of unidirectional channels which requires a single signature from the sender to authorise a payment. 
Notably, the unidirectional channels in Duplex can exhaust their supply of coins.
This requires both parties to co-operatively perform $(\alpha + 1) \times 2$ signatures to reset the coins in each channel, where $\alpha$ represents the list of transactions that need to be replaced in Invalidation Tree's current branch.

However, Raiden's unidirectional channels does not require a reset as it only increments the total quantity of transferred coins and an offset is considered during the settlement phase to compute the final balance for both parties. 

On the other hand, Lightning and Sprite maintain both party's current balance and sending a payment requires both parties to co-operatively sign a new transaction that updates their balances. 
Notably, Lightning revokes the previous state after both parties mutually agree a new state. 
These previous states are invalidated using a penalty approach that requires parties to store all pre-images $(x_{1},...,x_{n})$ and $(s_{1},...,s_{n})$. This storage requirement is highlighted in Table \ref{features} as $O(N)$, where $N$ is the number of previous states. 
On the other hand, Sprite increments a nonce which the contract enforces to represent the latest state. 

\textbf{Settlement and Dispute.}
All protocols can be settled if both parties co-operatively sign a transaction that sends them their final balance.

Duplex and Raiden potentially require the most on-chain transactions in the event of a dispute. 
In Duplex, the disputer should already have the signatures for all $d$ nodes in the current branch of the Invalidation Tree.
Both parties must sign the unidirectional channels that represent their latest payment from the counterparty and send both transactions to the network. 
In Raiden\footnote{Raiden have fixed a bug we reported during our analysis of their implementation \url{https://github.com/ raiden-network/raiden/issues/365}.}, each party signs the unidirectional channel that represents the latest payment from the counterparty and again two transactions are stored in the Blockchain 
However, each conditional transfer that needs to be unlocked requires the receiver to sign an additional transaction $\beta$ to claim it. 

Lightning requires the disputer to sign and send their Commitment Transaction for acceptance into the Blockchain.
It is possible for each party to sign a single transaction that claims both their final balance and all unlocked conditional transfers. 
However, depending on the lock times associated with the conditional transfers, then it is likely that an additional transaction $\beta$ is required to claim each conditional transfer.  

Unlike all others protocols, \textbf{Sprite is the only payment channel protocol that does not need to close in order to resolve a dispute for a conditional transfer}. 
Any party in the route can submit the pre-image $x$ of the conditional hash $H(x)$ to the PreimageManager.
This dispute will enforce the conditional transfer confirmation all channels if the preimage is accepted before the expiry time $T_{Expiry}$. 
Furthermore, it is possible for both parties to withdraw coins from the channel by co-operatively signing a withdrawal transaction. 
This can be sent to the Blockchain for the coins to be released without the need to close the channel. 

%\subsection{Lightning}
%
%In our implementation, round numbers are used to ensure that the most-recent agreed-upon state can be enforced with higher priority than earlier states.
%
%This is significantly more difficult to express in Bitcoin UTXO scripts. Poon-Dryja channels provide an ingenious solution to this problem.
%
%However, this technique requires each party to store a potentially ever-accumulating list of ``spent secrets.'' A corrupt opponent may at any time close the channel, forcing the honest party to fetch one of these secrets in order to defend their collateral.


%\subsection{Raiden}
%
%
%Raiden does not have a whitepaper. We attempted to analyze the Raiden code with our desired properties in mind.
%Raiden is a work-in-progress, but Ethereum and python code can be viewed online, and an initial demonstration of multi-hop transactions.
%
%As far as we can tell, Raiden supports most of the features we identified, 
%
%Raiden does not provide privacy 
%
%
%
%
%
%Raiden and Duplex rely on a pair of unidirectional channels which allows both protocols to only require a single signature and transaction to send a payment.
%However, in Raiden there are two transactions and signatures to set up a bi-directional channel, whereas in Duplex both parties must sign a single 
%This allows both p
% for sending payments. 
%Each depositor in Raiden signs a new transaction 
%Only depositors in Raiden are required to sign a new transaction  each depositor to sign a new transaction and require a single signature 
%Raiden only requires the depositor to establ
%Raiden and Duplex rely on a pair of unidirectional channels for sending payments. 
%This allows both channels to only require a signature from the sender for every new payment, and for Raiden 
%Duplex requires the most signatures and transactions due to the need for an Invalidation Tree to invalidate previously authorised payments. 
%
%
%In Duplex the lock time for a conditional transfer needs to be larger than the current and all later payment channel's lifetime. Unfortunately, the life-time of these channels are expected to be large to reduce the need to periodically settle on the Blockchain and re-open the channel. As such, a petty node that withholds a conditional transfer effectively locks the bitcoins for the channel's remaining lifetime. 
%
%For Storage - in Duplex up to d + 1 transactions need to be stored. This includes the current active branch in the invalidation tree and one of the unidirectional channels, plus the counter-party signtures for these transactions. At the time of dispute the party can simply sign the transactions and broadcast them. 
%
%In a dispute - the entire branch and two unidirectional channels need to be broadcast to the Blockchain. 
%
%In Lighting, the lock time for a conditional transfer needs to consider both the grace period $\lambda$ that provides the counterparty time to claim these bitcoins if the conditional transfer was previously revoked, and a safety parameter $\Delta$ to provide sufficient time for the transaction to get in the Blockchain in the event of a dispute. The lock time (similarly to Duplex) should be larger than the incoming connection, and shorter for the outgoing connection. However - these lock times are expected to be relatively small as it does not consider the channel's overall lifetime (there is none). 
%
%In terms of storage - in Lighting - all preimages for the revocation hashes need to be stored to ensure that if an revoked state is broadcast to the network, then the non-broadcaster can issue a penalty. There are potential storage savings by pre-computing a two chain of hashses and revealing them in the reverse order as the new revocation hash. Furthermore, a single (i.e. the currently active) commitment transaction needs to be stored.
%
%In a dispute - in both the good and bad case (latest commitment transaction) - three transactions are stored in the Blockchain. 
%
%In Raiden, the lock times are similar to the Lightning Network approach. Each node's lock time needs is larger for the receiving, and smaller for the sending. 
%
%In terms of storage - only the latest unidirectional channel needs to be localled stored. 
%
%In a dispute - Both unidirectional channels need to be stored (using two transactions), and a transaction for each locked transfer. 
%
%In Sprite, the lock time for the conditional transfer in the best case is constant for all hops along the route. In the event of a dispute (or coming close to the channel timeout) an honest's node incentive is to send the pre-image to the all-agreed Preimage Manager. This has the effect of confirming the conditional transfer for ALL nodes along the route as opposed to the single channel. The lock time only needs to consider a short period for the conditional transfer to complete, and the period of time it takes to get into the Blockchain. 
%
%In a dispute - only a single transaction is stored in the Blockchain which includes the preimage of the hash. 
%
%In terms of storage - only the latest transaction needs to be stored by the party as the order of transactions is guaranteed using a nonce. 
%
%Here we identify the concrete 
%
%Note however that there remain other features. In particular, we do not support 
%
%Existing payment channel solutions can be expressed as a generic.
%
%Hearn's channels are pre-configured with a fixed payment time, .
%
%This can be modeled with a functionality that does not allow the recipient to pay. A dishonest party can force the payment to abort, resulting in the paying at a final time.
%
%Update function.



==> sections/full_simulation.tex <==
\section{Validating our simulation with comparison to Flare.}
\label{sec:validation}
Flare is a decentralized routing protocol.


==> sections/implementation_.tex <==
wooooo

==> sections/raiden.tex <==
In this section, we provide a short survey of related payment channels Duplex Micropayment Channels, Lightning Channels and Raiden. A comprehensive comparsion for Duplex Micropayment Channels and Lightning Channels is available here \cite{mccorry2016towards} and we use its notation for describing all protocols. 

\paragraph{Duplex Micropayment Channels} 

\begin{table*}[t]
\centering
\begin{tabular}{|ll|}
\hline
\multicolumn{2}{|l|}{\textbf{Channel Establishment:}} \tabularnewline
$A \rightarrow B$: & Funding input $\pi_{A}$ \tabularnewline
$B\rightarrow A$: & Funding $T^{F}$, Invalidation Tree's first branch $(T_{1,k},...,T_{d,k})$ and a signature $\sigma^{B \rightarrow A}_{B,i}$ for the channel $C^{B \rightarrow A}_{i}$ \tabularnewline
$A \rightarrow B$: & Signature $\sigma^{A \rightarrow B}_{A,i}$ for the channel $C^{A \rightarrow B}_{i}$ and a signature for each node in the branch $(\sigma^{1,k}_{A},...,\sigma^{d,k}_{A})$ \tabularnewline
$B \rightarrow A$: & Signature for each node in the branch $(\sigma^{1,k}_{B},...,\sigma^{d,k}_{B})$ and a signature $\sigma^{F}_{B}$ for the Funding $T^{F}$ \tabularnewline
$A \rightarrow N$: & Signed Funding $T^{F}$ \tabularnewline
\multicolumn{2}{|l|}{\textbf{Send a Payment:}} \tabularnewline
$A \rightarrow B$: & Signature $\sigma^{A \rightarrow B}_{A}$ for channel $C^{A \rightarrow B}$ \tabularnewline
\multicolumn{2}{|l|}{\textbf{Send a Conditional Transfer:}} \tabularnewline
$A \rightarrow B$: & Signature $\sigma^{A \rightarrow B}_{A}$ for channel $C^{A \rightarrow B}$ which has an additional conditional transfer (output) based on $H(x)$  \tabularnewline

\multicolumn{2}{|l|}{\textbf{Reset Channels:}} \tabularnewline
$A \rightarrow B$: & Next branch in the Invalidation Tree $(T_{1,k},...,T_{d,k-1})$ and a signature $\sigma^{A \rightarrow B}_{A,i+1}$ for the channel $C^{A \rightarrow B}_{i+1}$ \tabularnewline 
$B \rightarrow A$ & Signature for each node in the branch $(\sigma^{1,k}_{B},...,\sigma^{d,k-1}_{B})$ and a signature $\sigma^{B \rightarrow A}_{B,i+1}$ for the channel $C^{B \rightarrow A}_{i+1}$ \tabularnewline 
$A \rightarrow B$: &  Signature for each node in the branch $(\sigma^{1,k}_{A},...,\sigma^{d,k-1}_{A})$ \tabularnewline 
\multicolumn{2}{|l|}{\textbf{Close channel (Dispute):}} \tabularnewline
$A \rightarrow N$: &  Each signed node in the current branch $(T_{1,k},...,T_{d,k })$ and the signed channel $C^{A \rightarrow B}_{i}$  \tabularnewline 
$B \rightarrow N$: & The signed channel  $C^{B \rightarrow A}_{i}$  \tabularnewline 
\multicolumn{2}{|l|}{\textit{Note: Must wait until the leaf node's expiry time $T_{d,k}$ to settle both channels. }}  \tabularnewline
\multicolumn{2}{|l|}{\textbf{Close channel (Co-operative):}} \tabularnewline
$A \rightarrow C$: &  Signature $\sigma^{S}_{A}$ for Settlement $T^{S}$ \tabularnewline
$B \rightarrow N$: &  Signed Settlement $T^{S}$ \tabularnewline
\hline
\end{tabular}
\captionof{figure}{\label{tab:duplex} Duplex Micropayment Channels with two parties $A,B$ and the Bitcoin network $N$.  }
\vspace{-6mm}
\end{table*}

A proposal by Decker and Wattenhofer supports bi-directional payments.
Its goal is to extend the number of transfers possible compared to Spilman's channels \cite{spilman01} within the same lifetime. 
Structurally, it relies on a pair of unidirectional channels $C^{A \rightarrow B}, C^{B \rightarrow A}$ and an invalidation tree with a single active branch that represents the current pair of unidirectional channels. 
Each node in the tree is a transaction whose absolute lock time is equal or larger than its parent i.e. $(T_{1,99}, T_{2,100}, T_{3,100})$.   

Remarkably, lock times have a transient property such that reducing the lock time of a node in the branch will automatically invalidate all children nodes.
This invalidation is leveraged if either unidirectional channel exhausts its supply of coins.
Both parties co-operate to create a new pair of unidirectional channels with their new respective balance before signing a new subset of nodes  with smaller lock times to invalidate the previous active branch. 
Table \ref{tab:duplex} and the following will explain each stage: 

\textbf{Channel Establishment:} 
Both parties co-operate to construct an unsigned funding transaction $T^{F}$, the first branch of the invalidation tree $(T_{1,k},...,T_{d,k})$, where $d$ is the number of nodes in the tree and $k$ is an absolute lock time that is equal or greater than the previous node's lock time, and the two unidirectional channels $A \rightarrow B, B \rightarrow A$.
All transactions are mutually signed in the reverse order, and the funding transaction $T^{F}$ is sent to the Bitcoin network and stored in the Blockchain. 

\begin{table*}[t]
\centering
\begin{tabular}{|ll|}
\hline
\multicolumn{2}{|l|}{\textbf{Channel Establishment:}} \tabularnewline
$A \rightarrow B$: & Revocation hash $H(S_{A,i})$, Funding input $\pi_{A}$ \tabularnewline
$B\rightarrow A$: & Revocation hash $H(S_{B,i})$, Unsigned Funding $T^{F}$, Signature $\sigma^{C}_{B,i}$ for $A's$ Commitment $T^{C,A}_{i}$ \tabularnewline
$A \rightarrow B$: & Signatures $\sigma^{C}_{A,i}$ for $B's$ Commitment $T^{C,B}_{i}$ and $\sigma^{F}_{A}$ for Funding $T^{F}$ \tabularnewline
$B \rightarrow N$: & Signed Funding $T^{F}$ \tabularnewline

\multicolumn{2}{|l|}{\textbf{Send a Payment:}} \tabularnewline
$A \rightarrow B$: & New revocation hash $H(S_{A,i+1})$ \tabularnewline
$B \rightarrow A$: & New revocation hash $H(S_{B,i+1})$, Signature $\sigma^{C}_{B,i+1}$ for $A's$ new Commitment Tx $T^{C,A}_{i+1}$ \tabularnewline
$A \rightarrow B$: & Pre-image of previous revocation hash $S_{A,i}$, Signature $\sigma^{C}_{A,i+1}$ for $B's$ new Commitment $T^{C,B}_{i+1}$ \tabularnewline
$B \rightarrow A$: & Pre-image of previous revocation hash $S_{B,i}$ \tabularnewline

\multicolumn{2}{|l|}{\textbf{Send a Conditional Transfer:}} \tabularnewline
$A \rightarrow B$: & HTLC Output based on $H(x)$ \textit{(Sender's role)} \tabularnewline
$A \leftrightarrow B$: &  \textit{Repeat Send a Payment with additional HTLC Output} \tabularnewline

\multicolumn{2}{|l|}{\textbf{Close channel (Dispute):}} \tabularnewline
$A \rightarrow N$: &  Latest Commitment $T^{C}_{A}$ \textit{(Broadcaster)} \tabularnewline
$B \rightarrow N$: &  Delivery $T^{D}_{B}$ \textit{(Non-broadcaster claims balance)}  \tabularnewline
$A \rightarrow N$: &  Revocable Delivery $T^{RD}_{A}$ \textit{(Broadcaster  claims balance after time $t$)}  \tabularnewline
$B \rightarrow N$: &  HTLC Delivery $T^{HD}_{B}$ \textit{(Receiver claims locked coins by revealing $x$)}  \tabularnewline
$A \rightarrow N$: &  HTLC Refund Delivery $T^{HR}_{A}$ \textit{(Sender is refunded the locked coins after time $t^{expire}$)}  \tabularnewline


\multicolumn{2}{|l|}{\textbf{Close channel (Co-operative):}} \tabularnewline
$A \rightarrow C$: &  Signature $\sigma^{S}_{A}$ for Settlement $T^{S}$ \tabularnewline
$B \rightarrow N$: &  Signed Settlement $T^{S}$ \tabularnewline
\hline
\end{tabular}
\captionof{figure}{\label{tab:lightning} Lightning Channels with two parties $A,B$ and the Bitcoin network $N$.  }
\vspace{-6mm}
\end{table*}

\textbf{Send a Payment:}
The sender creates and signs a new payment transaction $T^{P}$ that re-distributes the coins in their unidirectional channel.
Effectively, this transaction increments the coins sent to the receiver and decrements the sender's share of coins. 
If either channel exhausts its supply of coins, then both parties must co-operate to reset the balance of both unidirectional channels.
To reset, both parties identify a node in the current active branch that has a lock time that is greater than its parent node. 

For example, the middle transaction $T_{2,100}$ in the branch $(T_{1,99}, T_{2,100}, T_{3,100})$ is the next available node to have its lock time reduced. 
Both parties construct a new branch $(T_{1,99}, T'_{2,99}, T'_{3,100})$ and unidirectional channels $A \rightarrow B, B \rightarrow A$ that represents each party's respective balance.
Crucially, these transactions are signed in the reverse order such that the unidirectionals channels are signed before $T'_{3,100}$ and $T'_{2,99}$. 
It is important to note that the first transaction $T_{1,99}$ does not need to be re-signed. 

\textbf{Send a Conditional Transfer:}
The sender creates a new payment transaction $T^{P}$ with an additional output that locks coins into the conditional transfer in their unidirectional channel. 
These coins can be claimed by the receiver if the pre-image $x$ of the hash $H(x)$ is revealed before time $t^{expire}$. 
On the other hand, the coins are refunded to the sender if the coins have not been claimed by $t^{expire}$. 


\textbf{Close Channel (dispute): }
Raising a dispute requires either party to wait for each node in the invalidation tree's absolute lock time to expire before it can be broadcast and accepted into the Blockchain.
Notably, the leaf node's $T_{d,k}$ has two outputs to represent each party's unidirectional channel. If a payment transaction $T^{P}$ that represents the final balance of the unidirectional channel is not accepted into the Blockchain before $t_{refund}$, then the channel's locked coins are returned to the sender. 

\textbf{Close Channel (co-operative): }
Both parties mutually sign a settlement $T^{S}$ that has no lock time and sends each party their respective balance. 
This sent transaction is sent to the network and accepted into the Blockchain to close the channel. 


\paragraph{Lightning Network} 

A proposal by Poon and Dryja that is composed of two components to support off-chain transactions.
The first is Lightning Channels that accepts deposits from two parties to support bi-directional payments without an expiry time. 
The second is Hashed Time-Locked Transactions (HTLC) that supports atomic transfers between two or more channels.

Combined, both components support the functionality required to build a payment network on Bitcoin.
The coins deposited in each Lightning Channel provides a payment network with its liquidity, while HTLC transactions provides a means for parties that do not share a direct channel to transact with each other. 

Before describing Lightning Channels it is important to note that invalidation of previous payments is performed using a penalty approach. 
There is a single active state that represents each party's balance in the channel and a list of previously revoked states.
Cruically, broadcasting a revoked state allows the non-broadcaster to steal all coins in the channel. 
As such, only the mutually agreed active state that represents both parties current balance should be broadcast to the Blockchain. 
Table \ref{tab:lightning} and the following will explain each stage: 

\textbf{Channel Establishment:} Both parties exchange new revocation hashes $H(S_{A,i}),H(S_{B,i})$, an agreed relative lock time $t$ and an unsigned Funding Transaction $T^{F}$. 
Next, each party creates, signs and sends the counterparty a Commitment Transaction $T^{C}$ that represents the channel's current state. 
Finally, the Funding Transaction can be signed $\sigma^{F}$ and accepted into the Blockchain once both parties have received their signed Commitment Transaction $T^{C,A},T^{C,B}$. 

\textbf{Sending a Payment:} 
Authorising a payment requires both parties to exchange new revocation hashes $H(S_{A,i+1}), H(S_{B,i+1})$ and sign a new pair of Commitment Transactions $T^{C,A}_{i+1},T^{C,B}_{i+1}$.
Next, both parties need to invaldiate the previous pair of Commitment Transactions which simply involves exchanging the previous revocation hashes pre-images $S_{A,i},S_{B,i}$. 

\begin{table*}[t]
\centering
\begin{tabular}{|ll|}
\hline
\multicolumn{2}{|l|}{\textbf{Channel Establishment:}} \tabularnewline
$A \rightarrow C$: & Counterparty $B$, settlement time $t^{settle}$, token $\alpha$ \tabularnewline
$A \rightarrow C$: & Deposit $d_{a}$ \textit{(repeatable)}\tabularnewline
$B \rightarrow C$: & Deposit $d_{b}$ \textit{(optional)} \tabularnewline

\multicolumn{2}{|l|}{\textbf{Send a Payment:}} \tabularnewline
$A \rightarrow B$: & Signature $\sigma^{P}_{A}$, total transferred $\lambda_{A}$, nonce $c_{A,i+1}$, locksroot $\Gamma_{A}\footnote{Technically, the receiver can compute this root using their list of pending conditional transfers.} $\footnote{Require only when a conditional payment is locked.} \tabularnewline
\multicolumn{2}{|l|}{Where $\sigma^{CT}_{A} = S_{sk_{a}}(\alpha, B, \lambda_{A}, \Gamma_{A}, c_{A,i+1})$.} \tabularnewline 

\multicolumn{2}{|l|}{\textbf{Send a Conditional Transfer:}} \tabularnewline
$A \rightarrow B$: & Signature $\sigma^{CT}_{A}$, total transferred $\lambda_{A}$, nonce $c_{A,i+1}$ locksroot $\Gamma_{A}$, locked transfer $\gamma_{A}$ \tabularnewline
 & hash $h_{A}$, expiration $t^{expire}_{A}$ \tabularnewline
\multicolumn{2}{|l|}{Where $\sigma_{A} = S_{sk_{B}}(\alpha, B, \lambda_{A}, \Gamma_{A}, c_{A,i+1})$.} \tabularnewline

\multicolumn{2}{|l|}{\textbf{Close channel:}} \tabularnewline
$A \rightarrow C$: &  Signature $\sigma_{B}$, total transferred $\lambda_{B}$, nonce $c_{B}$, locksroot $\Gamma_{B}$ \textit{(B's latest transfer)} \tabularnewline
$B \rightarrow C$: &  Signature $\sigma_{A}$, total transferred $\lambda_{A}$, nonce $c_{A}$, locksroot $\Gamma_{A}$ \textit{(A's latest transfer)} \tabularnewline
$A \rightarrow C$: &  Locked transfer  $\gamma_{B}$, secret $s_{B}$, merkle tree branch $\theta_{B}$ \textit{(unlock transfer, repeatable)} \tabularnewline
$B \rightarrow C$: &  Locked transfer  $\gamma_{A}$, secret $s_{A}$, merkle tree branch $\theta_{A}$ \textit{(unlock transfer, repeatable)} \tabularnewline
\multicolumn{2}{|l|}{\textbf{Withdraw:}} \tabularnewline
$A \rightarrow C$: &  Settlement after $t^{settle}$\tabularnewline

\hline
\end{tabular}
\captionof{figure}{\label{tab:raiden} Raiden with two parties $A,B$ and the smart contract $C$.}
%\vspace{-6mm}
\end{table*}


\textbf{Sending a Conditional Transfer:} 
A conditional payment requires each channel along the route to lock coins that are only released if a secret $x$ of $H(x)$ is revealed.
Locking the coins requires the sender to receive a hash $H(x)$ from the previous hop along the route, both parties to exchange new revocation hashes $H(S_{A,i+1}),H(S_{B,i+1})$, and both parties to sign a new pair of Commitment Transactions $T^{C,A}_{i+1},T^{C,B}_{i+1}$. 
Similarly to sending a payment, both parties need to exchange the previous revocation hashes pre-image $S_{A,i},S_{B,i}$ to revoke the previous active state. 

Cruically, both Commitment Transactions have an additional output that locks the sender's coins into the transfer.
These coins are sent to the receiver if $x$ is revealed, or refunded to the sender if the transfer has expired after time $t^{expire}$. 
Notably, this approach supports concurrent conditional transfers as only additional outputs are required to lock the coins. 

\textbf{Close Channel (Dispute):} 
Raising a dispute requires the disputer to broadcast their Commitment Transaction to the Blockchain.
The non-broadcaster can claim their coins immediately by signing a Delivery Transaction $T^{D}$, whereas the broadcaster must wait a mutually agreed grace period $t$ before claiming their coins using a Revocable Delivery Transaction $T^{RD}$.
If the broadcaster sends a previously revoked Commitment Transaction to the Blockchain, then the grace period $t$ provides the non-broadcaster time to issue a Breach Remedy Transaction $T^{BR}$ that steals the broadcaster's share of coins. 

\textbf{Close Channel (Co-operative):} 
Both parties sign a new Settlement Transaction $T^{S}$ that sends both parties their respective balances.
This single transaction is sent to the network and accepted into the Blockchain to close the channel. 

\begin{table*}
\centering
\makebox[0pt][c]{\parbox{1\textwidth}{%
    \begin{minipage}[b]{0.55\hsize}\centering
  %\caption{Number of signatures required in each step for the Payment Channels. We use $\times 2$ to highlight if both parties need to co-operate. $d$ is the number of nodes in the branch of Duplex's Invalidation Tree, $\alpha$ is the subset of nodes in the branch of Duplex's Invalidation Tree that need to be resigned, and $\beta$ represents each conditional transfer that is unlocked on-chain.}
  \caption{A comparison on the number of signatures required for each stage.
	       %Both parties signing the same transaction is represented as $\times 2$, 
	       %The number of nodes that need signed in Duplex's invalidation tree is represented by $d$, and a subset of nodes as $\alpha$. 
	       %The number of conditional transfers that need to be signed and unlocked is represented as $\beta$.  
           %$\times 2$ represents both parties signing the same transaction.   
           }\label{sigs}
  \vspace{25pt}
  \small
  \begin{tabular}{c|c|c|c|c|c} &
    \begin{rotate}{30} Establishment \end{rotate} &
    \begin{rotate}{30} Payment \end{rotate} &
    \begin{rotate}{30} Transfer \end{rotate} &
    \begin{rotate}{30} Reset \end{rotate} &
    \begin{rotate}{30} Dispute \end{rotate} \\
\hline
Duplex & $(d + 2) \times 2 $ & $1$ & $1$ & $(\alpha + 1) \times 2$ & $1 \times 2$  \\
Lightning & $2 \times 2$  & $1 \times 2$ & $1 \times 2$ & N/A & $3$ or $\beta + 3$  \\
Raiden  & $1$ or $2$   & $1$ & $1$ & N/A & $\beta + 2$  \\ 
\textbf{Sprite}  & \textbf{1 or 2}  & \textbf{1 $\times$ 2}  & \textbf{1 $\times$ 2} & \textbf{N/A} & \textbf{1}  \\
  \end{tabular}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.40\hsize}\centering
  \centering
    \caption{Payment Channel Features} \label{features}
    \small
    \vspace{25pt}
  \begin{tabular}{c|c|c|c|c} &
    \begin{rotate}{30} Bi-directional \end{rotate} &
    \begin{rotate}{30} Storage of previous states \end{rotate} &
    \begin{rotate}{30} Worst-case delay \end{rotate} &
    \begin{rotate}{30} Incremental \end{rotate} \\
\hline
Lightning~\cite{lightning} &
\CIRCLE     & $O(N)$ & $O(\ell\Delta)$ & \Circle \\
Duplex~\cite{duplexchannels} &
\LEFTcircle & $O(1)$ & $O(\ell\Delta)$ & \Circle \\
Raiden    & 
\CIRCLE     & $O(1)$ & $O(\ell\Delta)$ & \Circle \\
Our work  & 
\CIRCLE     & $O(1)$ & $O(\ell+\Delta)$ & \CIRCLE \\
  \end{tabular}
    \end{minipage}
    \hfill
}}
\end{table*}

\paragraph{Raiden}
It is inspired by the Lightning Network and is in active development to implement off-chain state channels for Ethereum. 
Table \ref{tab:raiden} and the following will explain each stage: 

\textbf{Channel Establishment:} A single party creates the channel by submitting the counterparty's Ethereum account $B$, and a settlement time $t^{settle}$ that provides a time window between closing the channel and settling its final balance. 
Both parties deposit tokens\footnote{A Raiden-specified asset.} into the contract if they are satisfied with the settlement time $t^{settle}$. 

\textbf{Sending a Payment:} 
An incremental counter $c$ is responsible for establishing the order of payments and each unidirectional channel $A \rightarrow B, B \rightarrow A$ has its own counter $c_{A,i},c_{B,i}$ respectfully. 
Each payment requires the sender to increment their total transferred $\lambda_{A}$ and the counter $c_{A,i+1}$ before signing the payment $\sigma^{P}_{A}$ using their Ethereum account's private key. 
Notably, the total transferred $\lambda$ value can be greater than the sender's deposit due to how the final balance is computed during the final settlement which we will present shortly. 
Also, the lock root $\Gamma$ is only included and signed if there are pending conditional transfers. 


\textbf{Sending a Conditional Transfer:} 
The sender computes a hash $h$, the locked transfer amount $\gamma$, the conditional transfer's expiration time $t ^{expire}$, the new lockroot $\Gamma$ and an incremented counter $c$. 
This message is signed $\sigma^{CT}_{A}$ using the sender's Ethereum account's private key and sent to the receiver. 
The lock root $\Gamma$ is the root of a merkle tree for all pending conditional transfers $\gamma_{1},...,\gamma_{n}$ and must be included in future payments until all conditional transfers $t^{expire}_{1},...,t^{expire}_{n}$ have expired. 

\textbf{Close Channel:} Either party can close the channel by submitting the latest transfer received from the counterparty.
%\footnote{We found a bug during our invetigation that allowed the closer to submit both the counterparty's latest transfer, and their own latest transfer. The closer could sign a new transfer that sends no tokens and increments the counter $c$. This effectively reverses all payments. https://github.com/raiden-network/raiden/issues/365.} 
This begins the settlement period $t^{settle}$ that provides a grace period for the counterparty to submit the latest transfer received from the closer.  
Furthermore, it provides time to unlock and claim each pending conditional transfer. 
This transfer can be claimed by submitting the locked transfer $\gamma$, the secret $s$ that is the pre-image of the hash $h$, and a merkle tree branch $\theta$ that proves the sender committed to this transfer under the condition that $s$ is revealed before the expiration time $t^{expire}$. 
Notably, the current implementation requires a new transaction to claim each conditional transfer. 


\textbf{Settlement:} As mentioned previously, the total transferred $\lambda$ can exceed each sender's deposit in the contract. 
Determining the final balance requires computing the offset of each total transferred using the following equations: 

$A_{balance} = d_{A} + (\lambda_{B}- \lambda_{A})$

$B_{balance} = d_{B} + (\lambda_{A}- \lambda_{B})$

Finally, the party that does not inform the contract to perform the settlement is sent their balance first, and the remaining tokens in the contract is sent to the caller. 

%\textbf{Observations.} Unlike Duplex Micropayment Channels, the unidirectional channel's in Raiden do not require a reset if either channel exhausts their supply of tokens. 
%Instead, the total transferred amount for both channels must cotinuously increase together and an offset\footnote{TODO: I need a better way to phrase this} is considered during the settlement period. 
%Furthermore, the contract does not need to be aware of expired conditional transfers while the channel's closing time window is open. 
%However, it remains unclear if not storing expired conditional transfers is beneficial compared to the computation required to verify a merkle tree branch for each claimed conditional transfers. 

